One Graph to Rule them All: Using NLP and Graph Neural Networks to analyse Tolkien's Legendarium

Natural Language Processing and Machine Learning have considerably advanced Computational Literary Studies. Similarly, the construction of co-occurrence networks of literary characters, and their analysis using methods from social network analysis and network science, have provided insights into the micro- and macro-level structure of literary texts. Combining these perspectives, in this work we study character networks extracted from a text corpus of J.R.R. Tolkien's Legendarium. We show that this perspective helps us to analyse and visualise the narrative style that characterises Tolkien's works. Addressing character classification, embedding and co-occurrence prediction, we further investigate the advantages of state-of-the-art Graph Neural Networks over a popular word embedding method. Our results highlight the large potential of graph learning in Computational Literary Studies.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = xelatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto


==> tables/lotr1_centralities_table.tex <==
\begin{tabular}{lllll}[h]
\toprule
{} &                   degree &               betweennes &                closeness &               eigevector \\
\midrule
1  &                    Bilbo &                    Bilbo &                    Bilbo &                    Bilbo \\
2  &                    Frodo &                    Frodo &                    Frodo &                    Frodo \\
3  &                    Elves &                     Otho &                     Otho &                    Elves \\
4  &                     Otho &                    Merry &                    Elves &                     Otho \\
5  &                    Merry &                    Elves &                  Gandalf &                  Gandalf \\
6  &                  Hobbits &                  Hobbits &                    Drogo &  Sackville-Bagginses \\
7  &                  Dwarves &                  Dwarves &  Sackville-Bagginses &                    Drogo \\
8  &                  Gandalf &                  Lobelia &                  Hobbits &                  Hobbits \\
9  &                    Drogo &                    Sting &                    Merry &                    Merry \\
10 &  Sackville-Bagginses &                   Pippin &                    Sting &                    Sting \\
11 &                  Lobelia &                  Gandalf &                   Gollum &                   Gollum \\
12 &                    Sting &                    Drogo &                   Elrond &                   Elrond \\
13 &                   Pippin &  Sackville-Bagginses &                     Orcs &                     Orcs \\
14 &                   Gollum &                   Gollum &                  Dwarves &                  Dwarves \\
15 &                   Elrond &                   Elrond &                  Lobelia &                  Lobelia \\
\bottomrule
\end{tabular}


==> tables/lotr2_centralities_table.tex <==
\begin{tabular}{lllll}
\toprule
{} &      degree &  betweennes &   closeness &  eigevector \\
\midrule
1  &     Aragorn &     Aragorn &     Aragorn &     Aragorn \\
2  &     Gandalf &     Gandalf &     Gandalf &     Gandalf \\
3  &       Frodo &       Frodo &       Frodo &       Frodo \\
4  &  Sam Gamgee &  Sam Gamgee &      Pippin &  Sam Gamgee \\
5  &      Pippin &     Saruman &       Merry &      Pippin \\
6  &     Saruman &   Treebeard &  Sam Gamgee &       Merry \\
7  &     Faramir &      Pippin &     Saruman &     Boromir \\
8  &       Gimli &       Gimli &    the Orcs &     Faramir \\
9  &       Merry &    the Orcs &       Gimli &     Saruman \\
10 &    the Orcs &     Legolas &     Boromir &       Gimli \\
11 &   Treebeard &     Shagrat &     Faramir &    the Orcs \\
12 &     Boromir &     Théoden &   Treebeard &   Galadriel \\
13 &       Eomer &     Faramir &     Legolas &   Treebeard \\
14 &      Gollum &       Merry &   Galadriel &     Legolas \\
15 &     Legolas &       Elves &      Gollum &       Eomer \\
\bottomrule
\end{tabular}


==> tables/lotr3_centralities_table.tex <==
\begin{tabular}{lllll}
\toprule
{} &      degree &  betweennes &   closeness &  eigevector \\
\midrule
1  &     Aragorn &      Sauron &     Aragorn &     Aragorn \\
2  &      Pippin &     Aragorn &      Sauron &      Pippin \\
3  &     Gandalf &  Sam Gamgee &      Pippin &     Gandalf \\
4  &      Sauron &      Pippin &     Gandalf &      Sauron \\
5  &     Legolas &     Théoden &     Legolas &     Legolas \\
6  &       Gimli &     Gandalf &       Gimli &       Gimli \\
7  &       Merry &       Merry &    the Dead &    the Dead \\
8  &    the Dead &       Frodo &  Sam Gamgee &       Frodo \\
9  &     Théoden &       Gimli &       Frodo &     Imrahil \\
10 &  Sam Gamgee &     Legolas &    Denethor &      Elrond \\
11 &       Frodo &    Denethor &       Merry &  Sam Gamgee \\
12 &    Denethor &     Shagrat &     Imrahil &       Merry \\
13 &     Faramir &    Halbarad &    Beregond &    Denethor \\
14 &      Elrond &    the Dead &     Théoden &    Beregond \\
15 &     Imrahil &     Faramir &      Elrond &     Théoden \\
\bottomrule
\end{tabular}


==> tables/lotr3_centralities_table_main.tex <==

% \resizebox{.35\textwidth}{.15\textwidth} % .14\textwidth
% {
 \footnotesize
\begin{tabular}{llll}
\toprule
{} &      degree &  betweennes \\
\midrule
1  &     Aragorn &      Sauron  \\
2  &      Pippin &     Aragorn  \\
3  &     Gandalf &         Sam  \\
4  &      Sauron &      Pippin  \\
5  &     Legolas &     Théoden  \\
6  &       Gimli &     Gandalf  \\
7  &       Merry &       Merry  \\
8  &    the Dead &       Frodo  \\
9  &     Théoden &     Legolas \\
10 &         Sam &       Gimli \\
11 &       Frodo &    Denethor \\
12 &    Denethor &     Shagrat \\
13 &     Faramir &    Halbarad \\
14 &      Elrond &    the Dead \\
15 &     Imrahil &     Faramir \\
\bottomrule
\end{tabular}
% }

